Remote Sensing Change Detection via Weak Temporal Supervision

Semantic change detection in remote sensing aims to identify land cover changes between bi-temporal image pairs. Progress in this area has been limited by the scarcity of annotated datasets, as pixel-level annotation is costly and time-consuming. To address this, recent methods leverage synthetic data or generate artificial change pairs, but transferring change detection models across datasets and acquisition conditions remains challenging. In this work, we introduce a weak temporal supervision strategy that leverages additional temporal observations of existing single-temporal datasets, without requiring any new annotations. Specifically, we extend single-date remote sensing datasets with new observations acquired at different times and train a change detection model by assuming that real bi-temporal pairs mostly contain no change, while pairing images from different locations to generate change examples. To handle the inherent noise in these weak labels, we employ an object-aware change map generation and an iterative refinement process. We validate our approach on extended versions of the FLAIR and IAILD aerial datasets, showing competitive zero-shot and low-data regime performance. Lastly, we showcase results over large areas in France, highlighting the scalability potential of our method.

==> tables/main_results.tex <==
\makeatletter
\global\let\oriCT@@do@color\CT@@do@color

\begin{table*}[t!]
  \renewcommand{\arraystretch}{0.92}
  \caption{\textbf{Comparison with baselines.} For each data source, the best-performing results are shown in \textbf{bold}. Second-best results are \underline{underlined}. Note that SyntheWorld is a fully synthetic dataset, in contrast to FSC-180k or Changen2-S19-180k, which are built on FLAIR; therefore, evaluation on real data is always out-of-domain for models trained on SyntheWorld. $^\dagger$Results from~\cite{benidir2025change}.}
  \vspace{-2mm}
  \centering  
  \resizebox{0.95\linewidth}{!}{
  \begin{tabular}{cccccccccccccccccc}
    \toprule
    \multirow{4}{*}{\rot[90]{Data source}} & \multirow{4}{*}{Model} & \multirow{4}{*}{\shortstack{Dataset\\extension}} & \multirow{4}{*}{\rot[90]{Bi-temporal}} & \multirow{4}{*}{\rot[90]{Post-classif.}} & \multirow{4}{*}{\rot[90]{Synthetic~~~~}} & \multirow{4}{*}{\rot[90]{STAR~\cite{zheng2021change}{\tiny~~~}}} & \multirow{4}{*}{\rot[90]{Ours~~~~~~~~~~{\tiny~~}}} & \multicolumn{4}{c}{In-domain} & \multicolumn{6}{c}{Out-of-Domain}\\
    \cmidrule(lr){9-12}\cmidrule(lr){13-18}
    & & & & & & & & \multicolumn{2}{c}{FLAIR-BCD} & \multicolumn{2}{c}{FLAIR-BCD} & \multicolumn{2}{c}{LEVIR-CD} & \multicolumn{2}{c}{WHU-CD} & \multicolumn{2}{c}{S2Looking}\\
    & & & & & & & & \multicolumn{2}{c}{heldout} & \multicolumn{2}{c}{spot} &  &  & \\
    \cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}\cmidrule(lr){17-18}
    & & & & & & & & F1 & IoU & F1 & IoU & F1 & IoU & F1 & IoU & F1 & IoU \\
    \midrule
    \multirow{5}{*}{\rot[90]{FLAIR~~~~}} 
    & UNet      &   ---   & \xmark & \cmark & \xmark & \xmark & \xmark & 53.1 & 36.1 & --- & --- & 51.4 & 34.6 & 66.7 & 50.1 & 10.6 & 5.6 \\
    & UNet & b-FLAIR & \cmark & \cmark & \xmark & \xmark & \xmark & 51.9 & 35.0 & --- & --- & 40.3 & 25.3 & 65.6 & 48.8 & 8.8 & 4.6 \\
    & Dual UNet & Changen2-S19-180k~\cite{zheng2024changen2} & \xmark & \xmark & \cmark & \xmark & \xmark & 47.5 & 31.1 & --- & --- & \underline{51.8} & \underline{35.0} & 63.3 & 46.3 & \underline{13.4} & \underline{7.2}\\
    & Dual UNet & FSC-180k~\cite{benidir2025change} & \xmark & \xmark & \cmark & \xmark & \xmark & \textbf{77.7} & \textbf{63.5} & --- & --- & 49$^\dagger$ & 33$^\dagger$ & 63.3 & 46.3 & 4$^\dagger$ & 2$^\dagger$\\
    & Dual UNet &   ---   & \xmark & \xmark & \xmark & \cmark & \xmark & 55.8 & 38.7 & --- & --- & \textbf{53.3} & \textbf{36.3} & \underline{72.4} & \underline{56.7} & 11.8 & 6.3\\
    \rowcolor{blue!10}\global\let\CT@@do@color\relax & \global\let\CT@@do@color\oriCT@@do@color  Dual UNet & b-FLAIR & \cmark & \xmark & \xmark & \xmark & \cmark & \underline{68.7} & \underline{52.3} & --- & --- & 44.7 & 28.9 & \textbf{77.3} & \textbf{63.0} & \textbf{13.6} & \textbf{7.3} \\
    \midrule
    \multirow{5}{*}{\rot[90]{FLAIR-spot{\tiny~~}}} & \\
    & UNet      &      ---     & \xmark & \cmark & \xmark & \xmark & \xmark & --- & --- & 24.1 & 13.7 & 3.0 & 1.5 & 15.2 & 8.2 & 0.4 & 0.2 \\    
    & UNet      & b-FLAIR-spot & \cmark & \cmark & \xmark & \xmark & \xmark & --- & --- & \underline{25.0} & \underline{14.3} & \underline{19.5} & \underline{10.8} & \underline{28.6} & \underline{16.7} & \underline{1.9} & \underline{1.0} \\
    & Dual UNet &      ---     & \xmark & \xmark & \xmark & \cmark & \xmark & --- & --- & \textbf{29.2} & \textbf{17.1} & 0.7 & 0.4 & 5.2 & 2.7 & 0.1 & 0\\
    \rowcolor{blue!10}\global\let\CT@@do@color\relax & \global\let\CT@@do@color\oriCT@@do@color  Dual UNet & b-FLAIR-spot & \cmark & \xmark & \xmark & \xmark & \cmark & --- & --- & 22.9 & 12.9 & \textbf{34.1} & \textbf{20.6} & \textbf{49.3} & \textbf{32.7} & \textbf{7.1} & \textbf{3.7} \\
    \noalign{\vskip 3mm}
    \midrule
    \multirow{4}{*}{\rot[90]{IAILD~}}
    & UNet      &   ---   & \xmark & \cmark & \xmark & \xmark & \xmark & --- & --- & --- & --- & \underline{53.1} & \underline{36.2} &            42.6  &            27.1  &             4.6 &            2.4  \\
    & UNet      & b-IAILD & \cmark & \cmark & \xmark & \xmark & \xmark & --- & --- & --- & --- &            44.9  &            28.9  &            44.5  &            28.6  & \underline{7.9} & \underline{4.1} \\
    & Dual UNet &   ---   & \xmark & \xmark & \xmark & \cmark & \xmark & --- & --- & --- & --- &    \textbf{54.7} &    \textbf{37.6} & \underline{53.7} & \underline{36.7} &             6.1 &            3.1  \\
    \rowcolor{blue!10}\global\let\CT@@do@color\relax & \global\let\CT@@do@color\oriCT@@do@color  Dual UNet & b-IAILD & \cmark & \xmark & \xmark & \xmark & \cmark & --- & --- & --- & --- &            35.9  &            21.9  &    \textbf{63.3} &    \textbf{46.3} &    \textbf{17.6} &   \textbf{9.6} \\
    \midrule
    & Dual UNet & SyntheWorld~\cite{song2024syntheworld} & \xmark & \xmark & \cmark & \xmark & \xmark & --- & --- & --- & --- & 25$^\dagger$ & 13$^\dagger$ & 25.1 & 14.3 & 0$^\dagger$ & 0$^\dagger$\\
    \bottomrule
  \end{tabular}
  }
  \vspace{-.5em}
  \label{tab:comparison_results}
\end{table*}
